Algorithmic Fairness Verification with Graphical Models

In recent years, machine learning (ML) algorithms have been deployed in safety-critical and high-stake decision-making, where the fairness of algorithms is of paramount importance. Fairness in ML centers on detecting bias towards certain demographic populations induced by an ML classifier and proposes algorithmic solutions to mitigate the bias with respect to different fairness definitions. To this end, several fairness verifiers have been proposed that compute the bias in the prediction of an ML classifier--essentially beyond a finite dataset--given the probability distribution of input features. In the context of verifying linear classifiers, existing fairness verifiers are limited by accuracy due to imprecise modeling of correlations among features and scalability due to restrictive formulations of the classifiers as SSAT/SMT formulas or by sampling. In this paper, we propose an efficient fairness verifier, called FVGM, that encodes the correlations among features as a Bayesian network. In contrast to existing verifiers, FVGM proposes a stochastic subset-sum based approach for verifying linear classifiers. Experimentally, we show that FVGM leads to an accurate and scalable assessment for more diverse families of fairness-enhancing algorithms, fairness attacks, and group/causal fairness metrics than the state-of-the-art fairness verifiers. We also demonstrate that FVGM facilitates the computation of fairness influence functions as a stepping stone to detect the source of bias induced by subsets of features.

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%



==> tables/fairness_algorithms.tex <==

\begin{table*}       
    \centering
        \setlength{\tabcolsep}{.2em}
            \begin{tabular}{ll
            				ccc
            				ccc
            				ccc
            				ccc
            				ccc
            				ccc}
                \toprule
                \multirow{3}{*}{Encoding}& Dataset $ \rightarrow $   & 
                \multicolumn{8}{c}{Adult} &
%                \multicolumn{6}{c}{German} &
                \multicolumn{8}{c}{COMPAS} \\ 
                \cmidrule(lr){3-10}
                \cmidrule(lr){11-18}
                & Protected  $ \rightarrow $ & 
                \multicolumn{4}{c}{Race}   & \multicolumn{4}{c}{Sex}  &
%                \multicolumn{3}{c}{Age}   & \multicolumn{3}{c}{Sex}  &
                \multicolumn{4}{c}{Race}   & \multicolumn{4}{c}{Sex}
                \\ 
                \cmidrule(lr){3-6}
                \cmidrule(lr){7-10}
                \cmidrule(lr){11-14}
                \cmidrule(lr){15-18}

                 & Algorithm  $ \rightarrow $ &  
                orig. & RCO &
                orig. & CPP &
                orig. & RCO &
                orig. & CPP &
                orig. & RCO &
                orig. & CPP &
				orig. & RCO &
				orig. & CPP &
               \\
                \midrule
          
              
              
			Ind
			& DI&  $ 0.76 $ &  $ 0.67 $ &  $ 1.00 $ &  $ 0.71 $ &  $ 0.30 $ &  $ \mathbf{0.63} $ &  $ 1.00 $ &  $ 0.06 $ &  $ 0.96 $ &  $ 0.62 $ &  $ 1.00 $ &  $ \mathbf{1.00} $ &  $ 0.60 $ &  $ 0.55 $ &  $ 0.80 $ &  $ 0.75 $  \\
			& SP&  $ 0.15 $ &  $ 0.16 $ &  $ 0.00 $ &  $ 0.05 $ &  $ 0.53 $ &  $ \mathbf{0.21} $ &  $ 0.00 $ &  $ 0.13 $ &  $ 0.01 $ &  $ 0.14 $ &  $ 0.00 $ &  $ \mathbf{0.00} $ &  $ 0.13 $ &  $ \mathbf{0.13} $ &  $ 0.11 $ &  $ \mathbf{0.10} $  \\
			\midrule
			DAG
			& DI&  $ 0.73 $ &  $ 0.68 $ &  $ 1.00 $ &  $ 0.71 $ &  $ 0.33 $ &  $ \mathbf{0.68} $ &  $ 1.00 $ &  $ 0.05 $ &  $ 0.93 $ &  $ 0.62 $ &  $ 1.00 $ &  $ \mathbf{1.00} $ &  $ 0.62 $ &  $ 0.56 $ &  $ 0.80 $ &  $ 0.75 $  \\
			& SP&  $ 0.17 $ &  $ \mathbf{0.15} $ &  $ 0.00 $ &  $ 0.05 $ &  $ 0.51 $ &  $ \mathbf{0.17} $ &  $ 0.00 $ &  $ 0.15 $ &  $ 0.02 $ &  $ 0.14 $ &  $ 0.00 $ &  $ \mathbf{0.00} $ &  $ 0.13 $ &  $ \mathbf{0.13} $ &  $ 0.11 $ &  $ \mathbf{0.10} $  \\
			
			
               
            \bottomrule
    \end{tabular}
\caption{Logistic regression and two encodings: learn and learn-dependency. ``\textemdash'' refers to timeout of DAG learner (Notears). }
\end{table*}



\begin{table*}       
	\centering
	        \setlength{\tabcolsep}{.2em}
	\begin{tabular}{ll
			ccc
			ccc
			%            				ccc
			%            				ccc
			ccc
			ccc}
		\toprule
		\multirow{3}{*}{Classifier}& Dataset $ \rightarrow $   & 
		\multicolumn{6}{c}{Adult} &
		%                \multicolumn{6}{c}{German} &
		\multicolumn{6}{c}{COMPAS} \\ 
		\cmidrule(lr){3-8}
		\cmidrule(lr){9-14}
		%                \cmidrule(lr){15-20}
		& Protected  $ \rightarrow $ & 
		\multicolumn{3}{c}{Race}   & \multicolumn{3}{c}{Sex}  &
		%                \multicolumn{3}{c}{Age}   & \multicolumn{3}{c}{Sex}  &
		\multicolumn{3}{c}{Race}   & \multicolumn{3}{c}{Sex}
		\\ 
		\cmidrule(lr){3-5}
		\cmidrule(lr){6-8}
		\cmidrule(lr){9-11}
		\cmidrule(lr){12-14}
		%                \cmidrule(lr){15-17}
		%                \cmidrule(lr){18-20}
		
		& Algorithm  $ \rightarrow $ &  
		orig. & RW & OP & 
		orig. & RW & OP &
		%                orig. & RW & OP &
		%                orig. & RW & OP &
		orig. & RW & OP &
		orig. & RW & OP \\ 
		\midrule
		
		
		
		\multirow{3}{*}{\shortstack{Logistic \\ regression}}
		& Disparte impact&  $ 0.41 $ &  $ \mathbf{0.67} $ &  $ \mathbf{0.97} $ &  $ 0.04 $ &  $ \mathbf{1.00} $ &  $ \mathbf{0.76} $ &  $ 0.78 $ &  $ 0.49 $ &  $ 0.63 $ &  $ 0.64 $ &  $ 0.63 $ &  $ \mathbf{1.00} $  \\
		& Stat. parity&  $ 0.07 $ &  $ \mathbf{0.05} $ &  $ \mathbf{0.00} $ &  $ 0.16 $ &  $ \mathbf{0.00} $ &  $ \mathbf{0.02} $ &  $ 0.09 $ &  $ 0.31 $ &  $ 0.21 $ &  $ 0.16 $ &  $ 0.21 $ &  $ \mathbf{0.00} $  \\
		& Equalized odds&  $ 0.03 $ &  $ \mathbf{0.02} $ &  $ \mathbf{0.00} $ &  $ 0.08 $ &  $ \mathbf{0.00} $ &  $ \mathbf{0.06} $ &  $ 0.09 $ &  $ 0.31 $ &  $ 0.20 $ &  $ 0.17 $ &  $ 0.20 $ &  $ \mathbf{0.00} $  \\
		\midrule
		\multirow{3}{*}{\shortstack{Decision \\ tree}}
		& Disparte impact&  $ 0.65 $ &  $ \mathbf{1.00} $ &  $ \mathbf{0.80} $ &  $ 0.00 $ &  $ \mathbf{1.00} $ &  $ \mathbf{0.92} $ &  $ 0.96 $ &  $ \mathbf{0.97} $ &  $ \mathbf{1.00} $ &  $ 0.82 $ &  $ \mathbf{1.00} $ &  $ \mathbf{0.95} $  \\
		& Stat. parity&  $ 0.04 $ &  $ \mathbf{0.00} $ &  $ \mathbf{0.03} $ &  $ 0.17 $ &  $ \mathbf{0.00} $ &  $ \mathbf{0.01} $ &  $ 0.02 $ &  $ \mathbf{0.01} $ &  $ \mathbf{0.00} $ &  $ 0.07 $ &  $ \mathbf{0.00} $ &  $ \mathbf{0.02} $  \\
		& Equalized odds&  $ 0.12 $ &  $ \mathbf{-0.00} $ &  $ \mathbf{0.03} $ &  $ 0.45 $ &  $ \mathbf{0.00} $ &  $ \mathbf{0.06} $ &  $ 0.02 $ &  $ \mathbf{0.01} $ &  $ \mathbf{0.00} $ &  $ 0.07 $ &  $ \mathbf{0.00} $ &  $ \mathbf{0.06} $  \\
		
		
		
		
		
		
		
		
		\bottomrule
	\end{tabular}
	\caption{Verification of different fairness enhancing algorithms for multiple datasets and classifiers using {\framework}. Numbers in bold refer to fairness improvement  compared against the unprocessed (orig.) dataset. RW and OP refer to reweighing and optimized-preprocessing algorithm respectively. }
\end{table*}

==> tables/fairness_influence_functions.tex <==
\begin{figure}[h]
	\begin{center}
	
		\subfloat[COMPAS]{\includegraphics[scale=0.25]{figures/dependency_exp_Learn-dependency_compas_lr_sex_0}}
		\subfloat[COMPAS]{\includegraphics[scale=0.25]{figures/dependency_exp_Learn-dependency_compas_lr_sex_1}}
		\subfloat[COMPAS]{\includegraphics[scale=0.25]{figures/dependency_exp_Learn-dependency_compas_lr_sex_DI}}\\
		
		\subfloat[]{\includegraphics[scale=0.25]{figures/dependency_exp_Learn-dependency_adult_lr_sex_0}}
		\subfloat[]{\includegraphics[scale=0.25]{figures/dependency_exp_Learn-dependency_adult_lr_sex_1}}
		\subfloat[]{\includegraphics[scale=0.25]{figures/dependency_exp_Learn-dependency_adult_lr_sex_DI}}\\
		
	
		
	\end{center}
	\caption{Results on computing feature influence functions (FIF) for COMPAS  and Adult dataset.}
\end{figure}




==> tables/ssat_vs_subset_sum.tex <==

\begin{figure}
		\begin{center}
			\subfloat[]{\includegraphics[scale=0.25]{figures/ssat_vs_subsetsum_Independent_Adult_LR}}
			\subfloat[]{\includegraphics[scale=0.25]{figures/ssat_vs_subsetsum_DAG_Adult_LR}}
			\subfloat[]{\includegraphics[scale=0.25]{figures/ssat_vs_subsetsum_time_scatter_plot_Adult_LR}}\\
			
			\subfloat[]{\includegraphics[scale=0.25]{figures/ssat_vs_subsetsum_Independent_Adult_SVM}}
			\subfloat[]{\includegraphics[scale=0.25]{figures/ssat_vs_subsetsum_DAG_Adult_SVM}}
			\subfloat[]{\includegraphics[scale=0.25]{figures/ssat_vs_subsetsum_time_scatter_plot_Adult_SVM}}\\
			
			
			\subfloat[]{\includegraphics[scale=0.25]{figures/ssat_vs_subsetsum_Independent_Compas_LR}}
			\subfloat[]{\includegraphics[scale=0.25]{figures/ssat_vs_subsetsum_DAG_Compas_LR}}
			\subfloat[]{\includegraphics[scale=0.25]{figures/ssat_vs_subsetsum_time_scatter_plot_Compas_LR}}\\
			
			\subfloat[]{\includegraphics[scale=0.25]{figures/ssat_vs_subsetsum_Independent_Compas_SVM}}
			\subfloat[]{\includegraphics[scale=0.25]{figures/ssat_vs_subsetsum_DAG_Compas_SVM}}
			\subfloat[]{\includegraphics[scale=0.25]{figures/ssat_vs_subsetsum_time_scatter_plot_Compas_SVM}}\\
			
			\subfloat[]{\includegraphics[scale=0.25]{figures/ssat_vs_subsetsum_Independent_Ricci_LR}}
			\subfloat[]{\includegraphics[scale=0.25]{figures/ssat_vs_subsetsum_DAG_Ricci_LR}}
			\subfloat[]{\includegraphics[scale=0.25]{figures/ssat_vs_subsetsum_time_scatter_plot_Ricci_LR}}\\
			
			\subfloat[]{\includegraphics[scale=0.25]{figures/ssat_vs_subsetsum_Independent_Ricci_SVM}}
			\subfloat[]{\includegraphics[scale=0.25]{figures/ssat_vs_subsetsum_DAG_Ricci_SVM}}
			\subfloat[]{\includegraphics[scale=0.25]{figures/ssat_vs_subsetsum_time_scatter_plot_Ricci_SVM}}\\
			
			
			\subfloat[]{\includegraphics[scale=0.25]{figures/cactus_subsetsum_ssat_LR_time_.pdf}}
			\subfloat[]{\includegraphics[scale=0.25]{figures/cactus_subsetsum_ssat_SVM_time_.pdf}}
			

		\end{center}
		
		\caption{Scalability between {\framework} and Justicia. \red{Each instance represents the runtime of verifying on a dataset and a set of sensitive attributes.}}
\end{figure}
	
	
	


==> tables/verifier_scalability.tex <==
\clearpage

\begin{table}[t!]
    \centering
        \setlength{\tabcolsep}{.3em}
%        \vspace*{-.3em}
            \begin{tabular}{lrrrrrrrrrrrrrrr}
                \toprule
                Dataset   & \multicolumn{3}{c}{Ricci} & \multicolumn{3}{c}{Titanic} & \multicolumn{3}{c}{COMPAS} &  \multicolumn{3}{c}{Adult} &
                \multicolumn{3}{c}{German} \\ 
                
                \cmidrule(lll){2-4}
                \cmidrule(lr){5-7}
                \cmidrule(lr){8-10}
                \cmidrule(lr){11-13}
                \cmidrule(lr){14-16}
                

                Classifier & 
                LR & SVC & DT &
                LR & SVC & DT &
                LR & SVC & DT &
                LR & SVC & DT &
                LR & SVC & DT \\
				 \midrule

{\framework} &  $ \textbf{0.1} $  &  $ \textbf{0.1} $  &  $ \textbf{0.1} $  &  $ \textbf{0.1} $  &  $ \textbf{0.1} $  &  $ 1.6 $  &  $ \textbf{0.4} $  &  $ \textbf{0.5} $  &  $ 121.7 $  &  $ \textbf{0.9} $  &  $ 1.8 $  &  $ \textbf{0.3} $  &  $ \textbf{1.4} $  &  $ \textbf{1.4} $  &  $ 2.3 $  \\ 
Justicia &  $ 2.2 $  &  $ 2.2 $  &  $ \textbf{0.1} $  &  $ 0.3 $  &  $ 0.2 $  &  $ \textbf{0.3} $  & \textemdash & \textemdash &  $ \textbf{0.3} $  & \textemdash &  $ \textbf{1.7} $  &  $ 0.4 $  & \textemdash & \textemdash &  $ \textbf{0.2} $  \\ 
VeriFair &  $ 2.0 $  &  $ 1.8 $  &  $ 1.9 $  &  $ 0.5 $  &  $ 0.4 $  &  $ 17.2 $  &  $ 12.2 $  &  $ 11.6 $  &  $ 377.1 $  &  $ 7.3 $  &  $ 21.7 $  &  $ 57.9 $  &  $ 19.2 $  &  $ 28.8 $  &  $ 78.5 $  \\ 
FairSquare & \textemdash & \textemdash &  $ 4.6 $  & \textemdash & \textemdash &  $ 432.9 $  & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash \\ 



















	
		
			
				
				
				
				
				
				
				


    \end{tabular}
\caption{Scalability of different verifiers in terms of execution time (in seconds).  DT and LR refer to decision tree and logistic regression respectively. `\textemdash'~ refers to timeout. \red{Restricted experiments with Boolean single sensitive attribute.}}
\label{tab:FS_VF_Justicia}
%\vspace*{-1em}
\end{table}








\begin{table}[t!]
	\centering
	\setlength{\tabcolsep}{.3em}
	%        \vspace*{-.3em}
	\begin{tabular}{lrrrrrrrrrrrrrrr}
		\toprule
		Dataset   & \multicolumn{3}{c}{Ricci} & \multicolumn{3}{c}{Titanic} & \multicolumn{3}{c}{COMPAS} &  \multicolumn{3}{c}{Adult} &
		\multicolumn{3}{c}{German} \\ 
		
		\cmidrule(lr){2-4}
		\cmidrule(lr){5-7}
		\cmidrule(lr){8-10}
		\cmidrule(lr){11-13}
		
		
		Classifier & 
		LR & SVC & DT &
		LR & SVC & DT &
		LR & SVC & DT &
		LR & SVC & DT &
		LR & SVC & DT \\
		\midrule
		
		{\framework} &  $ 0.86 $  &  $ 1.0 $  &  $ 1.0 $  &  $ 0.16 $  &  $ 0.0 $  &  $ 0.59 $  &  $ 0.74 $  &  $ 0.85 $  &  $ 0.94 $  &  $ 0.65 $  &  $ 1.0 $  &  $ 0.49 $  &  $ 0.82 $  &  $ 0.9 $  &  $ 0.94 $  \\ 
		Justicia &  $ 0.26 $  &  $ 0.36 $  &  $ 0.3 $  &  $ 0.14 $  &  $ 0.0 $  &  $ 0.55 $  & \textemdash & \textemdash &  $ 0.79 $  & \textemdash &  $ 0.85 $  &  $ 0.22 $  & \textemdash & \textemdash &  $ 0.89 $  \\ 
		VeriFair &  $ 0.28 $  &  $ 0.4 $  &  $ 0.49 $  &  $ 0.1 $  &  $ 0.0 $  &  $ 0.87 $  &  $ 0.79 $  &  $ 0.74 $  &  $ 0.97 $  &  $ 0.79 $  &  $ 0.88 $  &  $ 0.93 $  &  $ 0.66 $  &  $ 0.64 $  &  $ 0.89 $  \\ 
		FairSquare & \textemdash & \textemdash &  $ 0.52 $  & \textemdash & \textemdash &  $ 0.87 $  & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash \\ 
		
		
		
		
		
		
		
		
		
		
		
		
		
		
		
	\end{tabular}
	\caption{Computed disparate impact by different fairness verifiers on different datasets and classifiers.  DT and LR refer to decision tree and logistic regression respectively. `\textemdash'~ refers to timeout.}
	\label{tab:FS_VF_Justicia}
	%\vspace*{-1em}
\end{table}
